An Evaluation of Cryptocurrency Payment Channel Networks and Their Privacy Implications

Cryptocurrencies redefined how money can be stored and transferred among users. However, independent of the amount being sent, public blockchain-based cryptocurrencies suffer from high transaction waiting times and fees. These drawbacks hinder the wide use of cryptocurrencies by masses. To address these challenges, payment channel network concept is touted as the most viable solution to be used for micro-payments. The idea is exchanging the ownership of money by keeping the state of the accounts locally. The users inform the blockchain rarely, which decreases the load on the blockchain. Specifically, payment channel networks can provide transaction approvals in seconds by charging a nominal fee proportional to the payment amount. Such attraction on payment channel networks inspired many recent studies which focus on how to design them and allocate channels such that the transactions will be secure and efficient. However, as payment channel networks are emerging and reaching large number of users, privacy issues are becoming more relevant that raise concerns about exposing not only individual habits but also businesses' revenues. In this paper, we first propose a categorization of the existing payment networks formed on top of blockchain-backed cryptocurrencies. After discussing several emerging attacks on user/business privacy in these payment channel networks, we qualitatively evaluate them based on a number of privacy metrics that relate to our case. Based on the discussions on the strengths and weaknesses of the approaches, we offer possible directions for research for the future of privacy based payment channel networks.

==> CoinExpress.tex <==
CoinExpress is another novel probing-based dynamic routing mechanism. It efficiently obtains “express lanes” in a cryptopayment network. Initially, CoinExpress concentrates on payment routing mechanism with high-performance capability and high-efficiency, while leaving the privacy issue as future work.  In CoinExpress, the sender inquiries for channel states before the payment and reserves balances \cite{yu2018coinexpress}. 

Being entirely distributed and adaptive to network dynamics, CoinExpress achieves a high goodput. It uses the Distributed breadth-first-search (BFS) algorithm to explore the augmenting paths for the transaction. CoinExpress has two different versions: CnExp-W, which selects the wides path for the payment, and CnExp-S with shortest path selection.

\subsubsection{System Model}

A distributed PCN is modeled as a weighted directed graph $G = (V; E)$. where $V$ represents the set of nodes and $E$ represents the set of links. A link can be unidirectional channel, from one transferor to transferee, as well as one direction of a bidirectional channel. Each link holds numerous attributes. 

First of all, each link $e \in E$ has a capacity for the channel, $c_e$, indicating the cumulative amount of value saved into the specific payment channel by both parties. Secondly, each link $e \in E$ also possesses a current \textit{balance} denoted by $b_e$. Let $G$ be a unidirectional channel, expressed by a one-way link, the capacity $c_e$ is the maximum amount of payment that the sender can send to the receiver before the channel deadline. Besides, the balance of $b_e$ is the remaining amount of value that the sender can send. 

Again, for a bidirectional channel where two collateral links are in opposite directions between two users, the two links possess the similar capacity, equal to the summation of their balances, expressed as, $b_{(u,v)} + b_{(v,u)} = c_{(u,v)} = c_{(v,u)}$. A link $e$ always has the specific balances and capacity $b_e \le c_e$. In general, we consider the set $E$ includes links with positive balances at any given time.  If any link has zero balances, it is temporarily removed from the network graph. Whenever a new deposit occurs in the opposite direction, the balance gets recharged, and the link becomes online again. 

Payment through a channel follows several steps to be completed. First, each channel requires to perform arriving payments sequentially. Second, it needs the forward processing time of the current hop. The time is necessary for the two parties to agree on the balance update. Third, due to the time lock in HTLC, whenever the channel receives the acknowledgment from the next hop, it releases the locked transferred value.  This one also requires a specified amount of waiting and backward processing time. 

For the simplification, the transmission delay between parties is ignored, considering that it is merged into the forward and backward processing times. In the model, $d^1_e$ is used to indicate the forward wait time along with the forward processing time of a link $e$ and $d^2_e$ to express the summation of backward wait time and the backward processing time. Thus, the total time, $d_e = d^1_e + d^2_e$. Each link has an expiration time denoted by $\eta_e$, expressing the time when a particular channel becomes unavailable. For payment via $e$ to be successful, it must settle before the channel expires. Only if the payment is completed before the deadline of the channel, it becomes successful. 


The proposed model assumed that every user only has the local knowledge on all its incoming and outgoing links. The knowledge includes their capacities, expiration times, balances, and delays.
The addresses of the sender and the receiver are shared among each other. However, the location in the network remains confidential. In general, every node may have an approximate estimation of the total network status based on the locally collected information. However, due to network asynchrony and dynamics, the instantaneous balance and delay of the remote nodes remain unknown. 


\subsubsection{Payment Model} In CoinExpress, any payment request is expressed by a quintuple $R = (s, t, a, st, dl)$, where $s$ is the sender, $t$ is the recipient, $a$ is the amount to be transferred, and $st$ and $dl$ are the start time and deadline for the payment respectively. Considering $\mathcal{P}$ as the set of all paths in the PCN. A payment request $R$ is obtained by a payment plan, consisting, a set of paths $P_R \in \mathcal{P}$, where each $p \in P_R$ is an $(s,t)$-path in the network. Each path  $p \in P_R$ is affiliated with a payment amount, indicated by $v_p$. For a payment plan $P_R$ to be successful, it needs to satisfy the following requirements:
 

 
\begin{itemize}
    \item $P_R$ is feasible, if and only if for any link $e \in E$ where $P_R(e) \subseteq P_R$ is the set of paths through $e$, thus
    $$
    \sum_{p \in P_{R}(e)} v_{p} \leq b_{e}
    $$
    
    \item $P_R$ is available, if and only if for any $p \in P_R$ and $e \in p$, let $p^{+}_ {e} \subseteq p$ be links including and after $e$ in $p$, then we have
    $$
    s t+\sum_{e \in p} d_{e}^{1}+\sum_{e \in p_{\epsilon}^{+}} d_{e}^{2} \leq \eta_{e}
    $$
    
    \item $P_R$ is timely, if and only if for any path $p \in P_R$, we have

    $$
    s t+\sum_{e \in p} d_{e} \leq d l
    $$
    
    \item $P_R$ is fulfilling, if and  only if

    $$
    \sum_{p \in P_{R}} v_{p} \geq a
    $$
\end{itemize}


With the light mentioned conditions, if a payment plan is  \textit{feasible, available, timely and fulfilling}, it can transfer $a$ amount of money from sender $s$ to recipient $t$ within the deadline $dl$. Only then it can be called as realizing payment plan for request $R$. The model aims at obtaining a realizing payment plan for each payment request while fulfilling as many goals as possible. The algorithm achieves much lower overhead with an excellent acceptance of goodput performance compared to all algorithms that consider user timeliness constraints.

==> Comp.tex <==


\begin{figure}[t]
\begin{center}
\includegraphics[width=\columnwidth]{Images/table1_SpeedyMurmus_SilentWhispers.png}
\caption{Performance of different transaction schemes in the static scenario, varying the routing algorithm}
\label{fig:SpeedyMurmus_SilentWhisper}
\end{center} 
\end{figure}

As expected, Ford-Fulkerson exhibited prohibitive delays and transaction overheads. tree-only routing finds the shortest route in the span- ning tree, possibly without passing a landmark, but does not include links that are not contained in the tree. Thus, tree- only routing is a compromise between SilentWhispers’ routing algorithm and embedding-based routing. As a consequence, the performance results when using only tree links are in between the performance of SilentWhispers and SpeedyMurmurs\par


They evaluate the impact of different configuration parameters on the performance. As indicated in the last two rows of Table 1, choosing random landmarks did not considerably affect the performance of SpeedyMurmurs but reduced the performance of Silent- Whispers due to the existence of longer paths to a landmark with few connections. The Fig:\ref{fig:Impact_of_number_of_parallel_trees_and_attempts_at_performing_a_transaction}shows the impact of number of parallel trees and attempts at performing a transaction. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=\columnwidth]{Images/Impact_of_number_of_parallel_trees_and_attempts_at_performing_a_transaction.png}
\caption{Comparing SpeedyMurmurs and SilentWhispers in a dynamic setting}
\label{fig:Impact_of_number_of_parallel_trees_and_attempts_at_performing_a_transaction}
\end{center} 
\end{figure}



The Fig:\ref{fig:SpeedyMurmus_SilentWhisper_dynamic} compares SpeedyMurmurs and SilentWhispers in a dynamic setting based upon Ripple transaction and link changes from 2013 to 2016 on per-epoch scale; success is computed as the ratio of the actual success ratio and the success ratio of the Ford-Fulkerson algorithm as a baseline; for c), we present moving averages over 50 epochs to increase readability



\begin{figure}[t]
\begin{center}
\includegraphics[width=\columnwidth]{Images/Comparing_SpeedyMurmurs_and_SilentWhispers_in_a_dynamic_setting.png}
\caption{Comparing SpeedyMurmurs and SilentWhispers in a dynamic setting}
\label{fig:SpeedyMurmus_SilentWhisper_dynamic}
\end{center} 
\end{figure}


According to the comparison, SpeedyMurmurs achieved higher performance than SilentWhispers concerning all considered metrics for the static scenario.On-demand stabilization and embedding-based routing had a positive effect on all 5-performance metrics. In contrast, the use of random credit assignment might decrease the success ratio slightly. However, when used in combination with embedding-based routing, the effect was mostly negated.As expected, Ford-Fulkerson usually achieved a higher success than both SpeedyMurmurs and SilentWhispers. However, the algorithm resulted in an enormous transaction overhead, exceeding the overhead of the other algorithms by 2 to 3 orders of magnitude.An increased number of trees or attempts to perform a transaction did not considerably increase the success ratio of SpeedyMurmurs but incurred increased overheads.The evolution of the PBT network affects the performance of SpeedyMurmurs considerably. Stabilization overhead and success ratio vary considerably depending on the frequency of transactions and link changes.


==> EE_P/PCN.tex <==
\textcolor{red}{BURADAN DEVAM EDIYORUZ}

\textcolor{red}{BURADAN DEVAM EDIYORUZ}

\textcolor{red}{BURADAN DEVAM EDIYORUZ}

\textcolor{red}{BURADAN DEVAM EDIYORUZ}

In the evolving world of trade, movement of money is going through changes and for a successful payment network is of great importance. To simply put, a payment network is a medium which is designed to move money from payer to payee. In the evolving world of payment networks the transacting (alet ne diyecegiz) unit can be not only money but it can be assets too. For the completeness of the paper we are interested in money movement. Other than cash payments there are 5 major payment systems with roots from going back to tens of years before today to a few years. These major payment systems are the paper checks, credit/debit cards, automated clearing house (ACH) payments, bank transfer and cryptocurrency based payments.

All of the methods other than the cryptocurrencies are controlled by 3rd party companies and regulated by the governments. Cryptocurrency backed payments are widely accepted as a liberation. The social, psychological, and economical impacts of cryptocurrencies are topics need to be extensively covered in other works, however, this paper aims elaborating how cryptocurrency based payment channel networks stand in the widely pervaded digital world.

\subsubsection{Credit Networks}

\subsubsection{Trust Networks}

\subsubsection{Social Networks}

\subsubsection{Payment Channel Networks}


HOW CAN WE DIfFERENYIATE THOSE?


target and equifax breach

==> Flare.tex <==
Flare\cite{prihodko2016flare} is another time-efficient hybrid payment routing protocol widely used in the lightning network. The primary goal of the protocol is to find the routes as quickly as possible. To obtain this goal, the nodes need to collect information from their neighboring nodes to estimate the topology of the lightning network. The collected information comprises both payment channels closer to the node in the node address space, considering hop distance and paths to beacon nodes. The combination of local and beacon nodes helps a node to reduce routing state while obtaining routes to any specific node with high probability.  The application of the beacon nodes helps to improve a node’s local view of the network with randomly chosen feeler nodes deeper inside the lightning network. Flare is highly scalable and can be implemented in a comprehensive network. The simulation results show that it performs perfectly even with 100,000 nodes. Fig. \ref{fig:flare_algo} shows the block diagram of the Flare algorithm.

\subsubsection{Model}

Considering the network as an undirected graph $G = (V, E)$, where $V$ represents the set of nodes and $E \subseteq V^2$ indicates the set of opened channels. 

For each channel $e \in E$, $Cap(e)$ is used to represent the total capacity of the channel. The authors consider binary symmetric function $Cap~:~ V^2 \rightarrow [0, + \infty)$, where capacity is 0 for any non-existant channel. 

$$\forall v_1,  v_2 \in V~~ (v1, v2)  \notin E \Leftrightarrow Cap(v_1, v_2) = 0$$


(Hop) distance between two nodes  is defined by the minimum number of channels in LN those connect those nodes:

$$d_{node}(x, y) := min\{n \in N:  \exists v_1,......., v_{n+1} \in V$$$$~~~x = v_1; y = v_{n+1} \forall i \in 1,.~.~., n ~~(v_i, v_{i+1}) \in E\}$$

Again, (Hop) distance between any node $x \in V$ and any channel $e = (y, z) \in E$ is defined by the minimum distance between the node and the channel’s ends:

$$d_{chan}(x, (y, z)) \equiv d_{chan}(x, e) : = min\{d_{node} (x, y),  d_{node} (x, z)\}$$
Adjacent nodes $Adj(v)$ for node $v \in V$ are determined by nodes at distance 1 :
$$Adj (v) = \{z \in V : d_{node} (v, z) = 1\}$$
In another way, adjacent nodes are those nodes with which $v$ has an opened payment channel.

A set of nodes, ($T$ ) is  connected by edges from the set of edges $T \subseteq E$:

$$Nodes (T ) : = \{ A : (A, ·) \in T \vee (·, A) \in T\}$$


Node addresses are used to ensure convergence of the routing algorithm. The node address is a node id which is unique though allover the network. It consists of a binary distance function established between all pairs of addresses. Each address is a 256-bit integer calculated as SHA-256 of the identity key of the node. Address distance between the nodes is an unsigned integer defined as bit-wise XOR of node addresses. 

\subsubsection{Routing Table}
To generate the routing table, Flare proposes another algorithm. 
Route discovery manages the node’s routing table. 

A routing table for a specidic node $v \in V$ includes a set of long
term (static) information about the LN topology: 
$$v.RT := \{(a_i, b_i) : (a_i; b_i) \in E\}$$
with the collection of payment channels $E$.

To store the routing table for each node, the following tasks are maintained:

\textit{Neighborhood map:} considers the channels between all node neighbors (considering hop distance) inside the neighbor radius $r_{nb} \in N$. This ensures that nodes separated from each other by no more than $2r_{nb}$ hops will get at least one route to each other.

\textit{Beacon paths:} consider the channels which form routes to $N_{bc}$ beacon nodes adjacent to the node in the address space. As node addresses are allocated randomly, each node having routes to other nodes are randomly scattered around the network.

\textit{Cached payment routes:} If any path is used by node earlier, it is saved in the chase memory. $N_{cache}$ channels that form paths to nodes that the node already used previously to complete payments. 
This saves time and helps the nodes learn working paths once they are considered in the reactive stage of the routing algorithm.

%_____________________________________
\begin{figure}[t]
\begin{center}
\includegraphics[width=\columnwidth]{Images/Flare.png}
\caption{Flare Algorithm}
\label{fig:flare_algo}
\end{center} 
\end{figure}
%__________________________________________

In the model, $x_p$ means the flow along route $p$ and $P = U_{i,j \in V} P_{i,j}$ is the collection of all paths. The capability limits of payment channels are indicated by the second set of constraints, and the third set of constraints express the balance condition. The balance constraints are essentially important for the flows calculated to be realizable.


\subsubsection{Neighborhood Discovery}
The neighbourhood information is updated based on several messages i.g. \textbf{NEIGHBOR\textunderscore HELLO},
\textbf{NEIGHBOR\textunderscore UPD}, \textbf{NEIGHBOR\textunderscore RST} and \textbf{NEIGHBOR\textunderscore ACK}, \textbf{NEIGHBOR\textunderscore HELLO}. 
\textbf{NEIGHBOR\textunderscore UPD} holds incremental adjustments to the node’s routing table since the most recent update message.
\textbf{NEIGHBOR\textunderscore RST} message is transmitted after update information was probably dropped.

\textbf{NEIGHBOR\textunderscore ACK} is used in response to \textbf{NEIGHBOR\textunderscore UPD} or \textbf{NEIGHBOR\textunderscore HELLO} to acknowledge that the node has appropriately received and processed the message.

\textit{Beacon Discovery} enables each node to find its neighborhood to expand its knowledge of the network. Beacons for node $u$, expressed as $u.bc \in V^{N_bc}$, are considered as the nearest nodes among the address space:

$$\forall v \in u.bc, \forall z \in V ~~\backslash~~ (\{u\} \cup u.bc) ~~~\rho (v, u) \lt \rho(z,u)$$
Beacon discovery is done using \textbf{BEACON\textunderscore REQ}, \textbf{BEACON\textunderscore ACK} and \textbf{BEACON\textunderscore SET} messages. \textbf{BEACON\textunderscore REQ} message is delivered to let the node know that it is opted as a beacon candidate. \textbf{BEACON\textunderscore ACK} message is used as a response and confirms that the node accepts to be a candidate. \textbf{BEACON\textunderscore SET} message is sent to inform that specific node that it is recognized as a beacon.


\subsection{Route Selection}
For route selection, the algorithm uses another two messages \textbf{TABLE\textunderscore REQ} and \textbf{TABLE\textunderscore RESP}. \textbf{TABLE\textunderscore REQ} is used to request for a routing table from the recipient. Besides, \textbf{TABLE\textunderscore RESP} is used in reply to \textbf{TABLE\textunderscore REQ} which contains a complete routing table of the sender.

\subsubsection{Ranking Candidate Routes} 
As soon as the routing algorithm finds a new route, the route is ranked based on its attributes and dynamic characteristics. To make it more efficient, both searching for the new route and ranking the found ones are done at the same time. Every time a new candidate route $p$ is found, the sender node starts its asynchronous ranking method, which calculates the route ranking $rr(p) \in [-\infty; +\infty)$.  The higher the ranking is, the better the route is. Ranking $-\infty$ indicates an unusable path. The author proposed a threshold for the well-ranked routers and if any routes have a ranking higher or equal to the rank, $r_{good}$; if $rr(p) \ge r_{good}$, it is selected as the final route. It reduces the duration of the routing algorithm.  

==> Flash.tex <==
 Flash\cite{wang2019flash} is a new dynamic routing solution, which makes use of the unique properties of transactions in offchain network, and makes a better compromise between path optimization and overhead detection. Flash performs high throughput and low overhead detection by dividing elephant payments from mice payments. Flash detects and finds candidate paths with sufficient capacity for elephant payments, and allocates the payments on these paths to minimize transaction fees by using an improved max-flow algorithm based on Edmonds Karp. Mice payments that can reduce the detection overhead are sent directly by finding the routing table with several precomputed paths.
Compared with the other routing algorithms, Flash has improved the success volume of payments at most 2.3x.\par

 
 \subsubsection{Architecture}Flash is a distributed online routing system. To achieve a better performance-overhead tradeoff, Flash separates elephant and mice payments and uses different routing algorithms. Flash first uses an improved maxi-flow algorithm to discover and detect the path with sufficient balance to meet its needs and then divides the payment path to minimize transaction fees by solving an optimization program. Flash uses a lightweight solution for Mice payments, which can be easily satisfied. If possible, it can route them randomly through a set of precomputed paths to reduce the detection overhead.\par
 
 Flash relays on two factors of offchain networks, one is the locally available topology. In the absence of channel balance information, the topology of the off-chain network is quite stable and changes every hour or every day. This is because opening or closing a payment channel takes at least several decades of on-chain transactions, while a channel usually remains in the network after it is established. Another one is the Atomic multipath payment. Flash uses multi-path routing as much as possible and assumes that the atomicity of multi-path payment is guaranteed, which is similar to the previous work. It also improved network utilization. Some mechanisms can achieve it, such as the Atomic Multi-path Payment (AMP) proposed for lightning. Based on HTLC, AMP allows split payments on multiple paths, while ensuring that recipients either receive all funds from multiple partial payments or receive nothing.\par
  %_____________________________________
\begin{figure}[t]
\begin{center}
\includegraphics[width=\columnwidth]{Images/flash_elephant_algorithm.png}
\caption{Modified Edmonds-Karp for elephant payment routing}
\label{fig:flash_algorithm}
\end{center} 
\end{figure}
%__________________________________________ 
  
 \subsubsection{Model}There are two models for Flash, one is an improved max-flow algorithm based on Edmonds-Karp using for elephant payments. Another one is a lightweight solution for mice payments\par
 
The network topology of every node that does not have capacity information. The sender $s$ uses the algorithm that shows in Fig: \ref{fig:flash_algorithm}  to route the elephant payment. The detected channel capacity of the paths can be recorded by using a matrix of the capacity $C$, and $C^'$ capacity matrix can record the unused capacity of channels that it is the same as Edmonds-Karp algorithm.  As shown in row 4 and 5 in Algorithm,  it initializes $C$ and $C^'$ to infinity. In the loop, it aims to find $k$ paths.  In row 7, Flash uses the BFS(Breadth-First-Search) to find a possible shortest path  $p$  that has an available value capacity, then add it to the set of the $ P$. The next step is to send detections of matrix $p$ to get the capacity of every channel and get the matrix $c$ of the bottleneck capacity.  Row 14 means send matrix $c$ on path matrix $p$. According to the results, $C_p $,  the detected capacity of channels and the remaining capacity can be updated. When the loop finishes, it will return the set of paths $P$ and the matrix of the capacity $C$ under the condition that the matrix $f$ of maxi-flow on certain paths has to satisfy the matrix $d$ of the payment demand.\par

For Elephant payments path selection in. Using a set of paths that got form the algorithm with sufficient capacity to minimize the transaction fees is another important step, and their information has collected in the algorithm. The below equation shows how to optimize it. The algorithm already provided the matrix $P$ of a set of paths and the matrix $C$ of the capacity.  A channel $(u,v)$ that has charging function $f_u_,_v$ can collect the fee information.  According to route a partial payment is  $r_p$ to $(u,v)$, the total fee is $f_u_,_v(r_p)$ if $f$ is convex. It aims to minimize the total fee under the constraints of meeting the payment demand of $d $ and respecting the channel capacity

\begin{itemize}
  
   \item $$
    min \sum_{p \in P} \sum_{_(_u_,_v_)} a_{u}^{P},_v f_u,(r_p)      
    $$ 
    \item 
    $$
    subject to \sum_{p \in P} r_p =d,
    $$
    \item 
    $$
   \sum_{p \in P}r_p a_{u}^{P}_,_v - \sum_{p \in P}r_p a_{v}^{P}_,_u \leq C(u,v), 	\forall(u,v).
    $$
\end{itemize}


\par
For Mice payments path finding, every node keeps a routing table that holds paths for the node receivers. If a new receiver is not in the routing table, the node will put shortest paths that calculated top-$m$ on the local topology matrix $G$  into the table.  Otherwise, Flash re-uses the existing paths. The Mice payments do not need a large routing table. Using top-$m$ shortest paths that matrix $m$ is extremely smaller than matrix $k$(used in the Elephant payments). The Mice payments show the performance better some times. The refreshment of the routing table is following the updating of the local network topology matrix $G$.\par

For Mice payments path selection. The sender decides the path to use a trial-and-error loop in the $m$ shortest paths of the routing table. If a sender sends a full payment using a random path $p$ successful, the transaction ends. Otherwise, the sender detects $p $ getting its effective capacity of $c_p $, and sends a part of the payment of volume $c_p $ within $p $.  The next step is updating the residual requirements for payment and keeps looping. This guarantees low detection overhead because flash only detects if it is necessary or up to $M $paths. The use of multi-path also improves the success rate of payment.\par
 
 


==> PA.tex <==
This section summarizes the different aspects of the routing protocols and performance. The metric used for the comparison is discussed below:

\subsubsection{Network}
The protocols are designed focusing the structure of different payment networks. The payment networks have both similarities and dissimilarities. As discussed in section \ref{CPN}, there is numerous cryptopayment network already implemented in real worked and some are proposed. The protocols are classified based on their corresponding network.
\subsubsection{Switching}
Any payment can be sent using a single transaction or it can be split in a few multiple small transactions. With the analogy of the traditional networking, if the payment is sent in a single transaction using a single route, then we calling the payment type as circuit switching. Otherwise, when the payment is divided into several smaller transactions and each transaction is sent through different paths, then this approach is analogous to the mechanism of packet switching. 
\subsubsection{Routing Algorithm}
There are a lot of algorithms used in the payment network models. Some protocols have their own/modified algorithm. Some protocols use the well established efficient algorithms as the backbone of the model. 
\subsubsection{Path}
The transactions can be one using an optimum path determined from the routing table. Otherwise, the transactions can be done using different distinct paths that connect the same sender and receiver. 
\subsubsection{Type of delivery}
The delivery can be two types in nature based on the amount sent. In atomic payment, the sender is only allowed to send the full amount or not at all. No fractional payment is accepted in the transactions. However, non-atomic payment allows us to send anything within the desired amount and the system accepts that fractional payment. Few protocols support only atomic payment while some support both.

\subsubsection{Privacy}
Privacy is one of the most important aspects of any routing protocol. Privacy must be preserved about the sender and receiver of the payment amount. Most of the algorithms do not consider privacy as an integrated part of the design, rather it leaves as a task of the other algorithms or as future work.\par


Table-\ref{tab:pa} shows the comparison of the routing protocols concerning different aspects. Fig: 3 shows the classification tree of the cryptopayment network protocols. The first classification is done on the switching category and the second one is based on consideration of privacy in the model.   


==> Silentwhisper.tex <==
The first distributed and privacy-preserving credit network routing algorithm is SilentWhispers. It does not need any entities to defend the integrity of the transactions. But, even in the face of untrusted users and malicious neighbors, SilentWhisperss can ensure the integrity and privacy of link values and transactions. SilentWhispers can also deal with network churn, which can be proved effective by using the payment data evaluation prototype extracted from the currently used Ripple payment network. \cite{malavolta2017silentwhispers}.\par

SilentWhispers uses a credit network design based on common landmark routing, which is a distributed setting. It can be extended by encryption structure and can do transaction between any two users while maintaining a strong privacy guarantee. SilentWhispers provides a new distributed payment protocol, which is used to calculate the available credit between the sender and receiver without revealing the credit information in related links or displaying transaction users. SilentWhispers allows users to be responsible for the correctness of credit updates. To improve its robustness,  the SilentWhispers has extended two features that include the offline nodes and security support. \par

\subsubsection{Architecture}

For routing, finding a path in the epochs is the major work. The routing information must be recalculated repeatedly to consider the dynamic nature of the credit network. Credit links between users are constantly updated, created and deleted due to transactions. Under the assumption that users are loose synchronization, the time should be divided into known periods. At the beginning of each period, a BFS tree and anti-tree should be created, and users use this routing information in the whole period.\par

For the credit on Path, the core technical challenge in the credit network design is to calculate the available credit on a specific path, which is necessary for the execution of transactions. First of all, a simple solution is to let each user in the path privately pass their link value to the corresponding landmark, so that the landmark can calculate the minimum value on the path and notify the expected receiver. However, it is easy to see that this approach does not guarantee the privacy of an honest but curious landmark because the landmark will get the credit associated with every link.\par

SilentWhispers has a local approach. The credit on the path is calculated step by step by every user in the path, which can not solve the privacy problem.  The protocol leaks all intermediate values when every user sends its value to the next in the path and receives a lower value from the previous user. Designing a secure multi-party computing (SMPC) protocol to calculate the available credit on the path is the basic idea of the approach. To improve  construction efficiency, landmarks play the role of calculators, and everyone gets a credit in every link from sender to receiver. Landmark can calculate the credit of the whole path intuitively by calculating a series of minimum functions, but it does not need to know any calculation results, of course, it does not need to know the credit of the link.\par

For constructing the path using a chained digital signature. The signature chain ensures all shares come from users, and from sender to receiver.  In a given path,  every user uses a long-term key pair to sign verification keys from their predecessors and successors. There is a result that a specific signature chain becomes a valid proof of the existence of the path from sender to receiver. However, combining long-term and fresh keys can improve the function. First, the user uses a long-term signature to sign a fresh verification key to bind them together. The long-term verification key is only displayed to the counterparty in the credit link, thus, the relationship between the fresh verification key and the user can verify the counterparty, but it is still hidden from other users in the credit network. Second, in any given path, the user can use the fresh signature key to sign the fresh verification key of the predecessor and successor to create a signature chain. For signatures checking, using the judge to determine the correctness of the value for the link. The long-term key is related to the identity of the real user so that the user is responsible for the behavior. \par


\subsubsection{Model}
The model uses $F_{CN}$ to intend the behaviors of the system, such as functionality, security, and privacy. For the ideal function of the credit network, $F_{CN}$ uses the matrix to maintain static information about nodes, links, and their credits locally. Also, $F_{CN}$ records all of the changes to the credits between nodes caused by successful transactions and we denote by $val^t_{u,u^'}$ the credit between some u and $u^'$ at time t. A set of functionalities of $F_{CN}$ includes $F_{ROUT}$, $F_{PAY}$, $F_{TEST}$, $F_{CHGLINK}$, $F_{TESTLINK}$, and $F_{ACC}$. $F_{CN}$ periodically performs functions to update the routing information of nodes in the network ($F_{ROUT}$) by using $F_{NET}$ as asynchronous means. Nodes can contact the ideal function to perform transactions ($F_{PAY}$), test available credits ($F_{TEST}$), update credits on links ($F_{CHGLINK}$), test credits on links ($F_{TESTLINK}$), or resolve disputes related to credits on certain links ($F_{ACC}$). \par

$F_{ROUT}$: $F_{ROUT}$ receives two tuples of the form ($u_1$, . . . , $u_m$) by LM. It is the sets of neighbors of LM in the tree and anti- tree, individually. It uses a BFS on the links to build the tree and anti-tree rooted at the landmark $ID_{LM}$. For every user $u$ belongs to the set, $F_{ROUT}$ sends a message $(sid, ID_{LM}, h, u_p )$ through $F_{SMT}$. $h$ is the amount of hops that divides $u$ from $ID_{LM}$. $u_p$ is the parent node on the path. $u$ gives $(\perp, sid)$, making $F_{ROUT}$  backward to the former user, $(u^{'}, sid)$ shows the next user $u^{'}$ adding into the set. The set is empty meaning the algorithm ends.\par

$F_{PAY}$: $F_{PAY}$ receives the tuple($S_{dr}$, $R_{vr}$, $T_{xid}$, $ID_{LM}$) from a sender. $S_{dr}$. $R_{vr}$, $T_{xid}$, and $ID_{LM}$ indicate the receiver. $F_{PAY}$ sends ($T_{xid}$, $ID_{LM}$, $u$) through $F_{SMT}$. $u$ is the preceding user in the chain. $F_{PAY}$ computes the set of tuples $P$={$ID_{LM}$,$v_{LM}$}. $v_{LM}$ is the credit connected by the path from the $S_{dr}$ to the $R_{vr}$ through LM ($path_{LM}$). $F_{PAY}$ sends ($P$, $T_{xid}$) to the $S_{dr}$ through $F_{SMT}$. $S_{dr}$ sends (\perp, $T_{xid}$) to $F_{PAY}$ or sends a set of tuples ($ID_{LM}$, $x_{LM}$, $T_{xid}$) to $F_{PAY}$ through $F_{SMT}$. $F_{PAY}$ sends($x_{LM}$, $ID_{LM}$ , $T_{xid}$) through $F_{SMT}$ to tell all the nodes in $path_{LM}$ of the value $x_{LM}$. $F_{PAY}$ sends $R_{vr}$ the tuple ($S_{dr}$, $R_{vr}$, $v$, $T_{xid}$) through $F_{SMT}$.  $v$ is the whole number transacted to $R_{vr}$. $R_{vr}$ sends (\perp, $T_{xid}$) or sends ($success$, $T_{xid}$).\par

$F_{ACC}$: Nodes $u_0$ and node $u_1$ sends the tuple ($val_0$,$u_0$,$u_0^'$), ($val_1$,$u_1$,$u_1^'$) respectively to contact $F_{ACC}$ through $F_{SMT}$. $F_{ACC}$ tests if $u_0^'$ = $u_1$ and $u_1^'$ = $u_0$. The next step is letting $t$ present the current time, iterating until $t$ = 0. $F_{ACC}$ queries $F_{CN}$ to retrieve $val^t_(_u_0_,_u_1_)$. If $val^t_(_u_0_,_u_1_)$ = $val_0$, then $F_{ACC}$ sends the tuple (0,$val_0$,$val_1$) to $u_0$ and $u_1$ through $F_{SMT}$. if $val^t_(_u_0_,_u_1_)$ = $val_1$, then the functionality sends the tuple (1, $val_0$ , $val_1$ ) to $u_0$ and $u_1$ through $F_{SMT}$. Otherwise, $F_{ACC}$ sets $t$ = $t$ -1. $F_{ACC}$ returns (\perp,$val_0$,$val_1$).



==> SpeedyMurmurs.tex <==
For decentralized PBT networks, SpeedyMurmurs is a new routing algorithm. It uses efficient and flexible embedding-based path discovery. It is efficient and stable on demand to deal with the dynamics of PBT networks. It reduces the stable overhead by two orders of magnitude, reduces the transaction routing fee by more than two times, maintains at least the same success rate as decentralized landmark routing, and provides low latency to get the key privacy goal of decentralized PBT network routing. \cite{roos2017settling}. \par

\subsubsection{Architecture}
SpeedyMurmurs considers both the available funds and the closeness to the destination of a neighbor when routing a payment, resulting in an efficient algorithm with flexible path selection. It utilizes an on-demand, efficient, stable algorithm that responds to changes in links when necessary, but maintains a low overhead corresponding to those changes. It enhances the processing of concurrent transactions by allowing nodes to actively and accurately allocate the funds needed for transactions, rather than prohibiting concurrent transactions from using links completely or taking the risk of failure in the subsequent payment phase. SpeedyMurmurs performs transactions about twice as fast as SilentWhispers, reducing transaction communication overhead by at least twice while maintaining similar or higher efficiency. It reduces the overhead of managing link changes by two to three orders of magnitude, except in rare periods when burst data sets correspond to sudden rapid growth. SpeedyMurmurs implements the privacy of value and the value of the transaction are kept hidden. The sender and receiver privacy is the identity of two users keeps hidden from the opponent.

\subsubsection{Model}
For distributed PBT network,  $(G, w)$ means a directed graph $G = (V, E)$. $w$ is a function of weight on the set of edges. The set of the nodes $V $ corresponds to the members of the PBT network. $u$ can transfer funds to $v$ if there is a link between $u$ to $v$. The set of outgoing neighbors of a node $v$ belongs $N_{out}(v) =  \{u \in V : (v,u) \in E\}$. The set of incoming neighbors of a node $v$ belongs $N_{in}(v) = \{u \in V :  (u, v) \in E \}$. A path $p$ is a sequence of links $e_1 ... e_k$ with $e_i = (v_i^1,v_i^2)$, and $v_i^2 = v^1_{(i+1)}$ for $1 \le i \le k-1$. $L = \{l_1,...,l_{|L|}\}$ represents a set of nodes, called landmarks,  well known to other users in the PBT network. $|L|$ represents the size of the set $L$.\par
$w$ defines the whole funds that can be transferred within two nodes sharing a link. The specific implementation of the function $w$ should be abstracted. For example, in the Bitcoin Lightning Network, the $ w: E \rightarrow  \mathrm{R}$ describe bitcoins $u$ can transfer to $v$ under an opening payment channel within them. The funds are available in a path $e_1,...,e_k$ as the $\textit{minimum} w(e_i)$. The net balance of a node $v$ belongs $cnode(v)= \sum_{u \in N_{in}(v)} w(u,v)- \sum_{u \in N_{out}(v)} w(v,u)$. \par

A tuple of algorithms (\textit{setRoutes, setCred, routePay}) are the conponments of a PBT network: \par

\textit{setRoutes(L)}: Provided the set $L = \{l_1, . . . , l_{|L|}\}$ of land- marks. In the PBT network, each node requires the routing information initialized by \textit{setRoutes}.\par

\textit{setCred(c,u,v):} Provided the value $c$, nodes $u$, and $v$. setCred sets $w(u,v) = c$. Moreover, \textit{setRoutes} initially generates the routing information may be changed by \textit{setCred}. \par

$((p_1,c_1),...,(p_{|L|}, c_{|L|})) \leftarrow routePay(c,u,v)$. Provided the value $c$,  $u$ and $v$, \textit{routePay} returns a set of tuples $(p_i , c_i )$, represent that $c_i$ funds are routed by the path defined by $p_i$.\par



%The Fig:\ref{fig:SpeedyMurmus_SilentWhisper} displays the results for different combinations of the three proposed modifications to SilentWhispers as well as our implementations of tree-only routing and Ford-Fulkerson


==> Spider.tex <==
Spider is a packet-switched network architecture in the cryptopayment network \cite{spider_small}. One of the principal goals of the routing algorithm is to maximize the throughput while inducing the channel balance. It has two distinct features that make the protocol different from others. Firstly, it splits a payment into several units and then make the transaction through different paths over a while. This procedure is similar to the approach of the packet switching algorithm in the standard data-based network. To attain high utilization of payment channel funds, it applies congestion control and in-network scheduling of transaction units. Besides, it supports both atomic and non-atomic payments with a deadline for each. \par 

The second specialty is the aware imbalance routing, which includes constraint for rate-imbalance routing to optimize throughput. The payment channel has price is both directions, which is updated locally based on the congestion control and imbalance in the network. Spider has a decentralized algorithm along with simple heuristic algorithms. Unlike other algorithms, spider considers the constraint to balance the channel imbalance as an integrated part of the algorithm. 
 
 \subsubsection{Architecture}
Being a packet-switched payment channel network, Spider hosts transfer payments through the system in series of transactions. The transaction units are always withing the maximum transaction unit (MTU). Individual transaction units pass though the spider routers as funds utilizing the payment channel. Each host runs a transport layer that incorporates standard facilities for applications to send and receive payments on the network. The application contains the destination address, the amount to be sent, a deadline, and the maximum allowable routing charge for every transaction.
The transport includes facilities for both atomic and non-atomic payments. Spider uses Atomic Multi-Path Payments (AMP) for the atomic payments. AMP breaks a payment into several transactions and sends it over different paths.  It also transmit the keys for all payment transaction units from a single base key. It makes sure that the receiver is not able to unlock any payment before getting all transaction units.   \par 

Similar to the Lightning Network, the authors also introduced the utilization of Onion routing to assure the privacy of user payments for any transaction unit. Queuing and waiting for transaction units at Spider routers could end up with unexpected delays for some payments. Nevertheless, the routers can allow distinct levels of service by scheduling transaction units depending on the payment specifications. It can prioritize payments based on volume, deadline, or routing expenses. 

\subsubsection{Model}

Let the payment channel network model be modeled as a graph $G(V, E)$. Here $V$ is the set of routers and $E$ is the set of payment channels.  For any pair of source and destination routers, denoted by $i,j \in V$ , let $d_{i,j} \ge 0$ express the regular rate at which transaction units is transported from $i$ to $j$. Besides, let $c_e$ be the total quantity of funds in channel $e$, for $e \in E$, and $\Delta$ is the usual latency faced by transaction units due to different types of network delays. Lastly let $P_{i,j}$ indicate the set of routes from $i$ to $j$ in $G$, for $i,j \in V$. Only ‘trails’, i.e., routes without repeated edges, in $P_{i,j}$ are included. Usually, any payment flow from source to destination routers maintain the demands $d_{i,j}$ as per fluid model. Usually, flow is expressed by a tuple with path and value. Here, path means the selected route and value means the payment conducted by the flow. Thus, the routing is calculated in a way that the average rate of money carried along the path matches the value of the flow.  Therefore, in the fluid model, maximizing throughput is similar to finding flows of maximum total value and can be expressed as a Linear Program (LP) as given in equation- 1.  

%_____________________________________
\begin{figure}[t]
\begin{center}
\includegraphics[width=\columnwidth]{Images/spider_algo.png}
\label{fig:spider_algo}
\end{center} 
\end{figure}


%__________________________________________

In the model, $x_p$ means the flow along route $p$ and $P = U_{i,j \in V} P_{i,j}$ is the collection of all paths. The capability limits of payment channels are indicated by the second set of constraints, and the third set of constraints express the balance condition. The balance constraints are essentially important for the flows calculated to be realizable.

==> tree.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\caption{Comparison of different routing protocols}
\label{tab:pa}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Protocols}              & \textbf{Network}             & \textbf{Switching} & \textbf{Algorithm}        & \textbf{Delivery}                                               & \textbf{Privacy} \\ \hline
\textit{\textbf{Spider}}        & Spider Network               & Packet Switching   & Water filling             & \begin{tabular}[c]{@{}l@{}}Atomic and\\ Non-atomic\end{tabular} & Not considered   \\ \hline
\textit{\textbf{CoinExpress}}   & Payment Channel Network      & Circuit Switching  & Ford-Fulkerson            & Atomic                                                          & Not considered   \\ \hline
\textit{\textbf{Flare}}         & Lightning Network            & Circuit Switching  & Landmark Routing          & Atomic                                                          & Not considered   \\ \hline
\textit{\textbf{Speedymurmur}}  & Decentralized PBT            & Circuit Switching  & Embedding-based Routing   & Atomic                                                          & Considered       \\ \hline
\textit{\textbf{SilentWhisper}} & Decentralized Credit Network & Packet Switching   & Landmark-centered Routing & Atomic                                                          & Considered       \\ \hline
\textit{\textbf{Flash}}         & Offchain Network             & Packet Switching   & Dynamic Routing           & Atomic                                                          & Not considered   \\ \hline
\end{tabular}%
}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
%_____________________________________
\begin{figure*}[h]
\label{fig:tree}
\centering
\includegraphics[trim=0cm 3.5cm 0cm 0cm, scale=0.5]{Images/Tree.pdf}
\caption{Classification tree of the routing protocols}
\end{figure*}
%__________________________________________
%%%%%%%%%%%%%%%%%%%%%%%%%
